No Conclusive Evidence for Transits of Proxima b in MOST photometry

The analysis of Proxima Centauri's radial velocities recently led Anglada-Escud\'e et al. (2016) to claim the presence of a low mass planet orbiting the Sun's nearest star once every 11.2 days. Although the a-priori probability that Proxima b transits its parent star is just 1.5%, the potential impact of such a discovery would be considerable. Independent of recent radial velocity efforts, we observed Proxima Centauri for 12.5 days in 2014 and 31 days in 2015 with the MOST space telescope. We report here that we cannot make a compelling case that Proxima b transits in our precise photometric time series. Imposing an informative prior on the period and phase, we do detect a candidate signal with the expected depth. However, perturbing the phase prior across 100 evenly spaced intervals reveals one strong false-positive and one weaker instance. We estimate a false-positive rate of at least a few percent and a much higher false-negative rate of 20-40%, likely caused by the very high flare rate of Proxima Centauri. Comparing our candidate signal to HATSouth ground-based photometry reveals that the signal is somewhat, but not conclusively, disfavored (1-2 sigmas) leading us to argue that the signal is most likely spurious. We expect that infrared photometric follow-up could more conclusively test the existence of this candidate signal, owing to the suppression of flare activity and the impressive infrared brightness of the parent star.

==> journals.tex <==
%\newcommand{\aj}{{\it AJ}}%
          % Astronomical Journal
\newcommand{\actaa}{{\it Acta Astron.}}%
          % Acta Astronomica
%\newcommand{\araa}{{\it ARA\&A}}%
          % Annual Review of Astron and Astrophys
%\newcommand{\apj}{{\it ApJ}}%
          % Astrophysical Journal
%\newcommand{\apjl}{{\it ApJ}}%
          % Astrophysical Journal, Letters
%\newcommand{\apjs}{{\it ApJS}}%
          % Astrophysical Journal, Supplement
%\newcommand{\ao}{{\it Appl.~Opt.}}%
          % Applied Optics
%\newcommand{\apss}{{\it Ap\&SS}}%
          % Astrophysics and Space Science
%\newcommand{\aap}{{\it A\&A}}%
          % Astronomy and Astrophysics
%\newcommand{\aapr}{{\it A\&A~Rev.}}%
          % Astronomy and Astrophysics Reviews
%\newcommand{\aaps}{{\it A\&AS}}%
          % Astronomy and Astrophysics, Supplement
%\newcommand{\azh}{{\it AZh}}%
          % Astronomicheskii Zhurnal
%\newcommand{\baas}{{\it BAAS}}%
          % Bulletin of the AAS
\newcommand{\caa}{{\it Chinese Astron. Astrophys.}}%
  % Chinese Astronomy and Astrophysics
\newcommand{\cjaa}{{\it Chinese J. Astron. Astrophys.}}%
  % Chinese Journal of Astronomy and Astrophysics
%\newcommand{\icarus}{{\it Icarus}}%
  % Icarus
\newcommand{\jcap}{{\it J. Cosmology Astropart. Phys.}}%
  % Journal of Cosmology and Astroparticle Physics
%\newcommand{\jrasc}{{\it JRASC}}%
          % Journal of the RAS of Canada
%\newcommand{\memras}{{\it MmRAS}}%
          % Memoirs of the RAS
%\newcommand{\mnras}{{\it MNRAS}}%
          % Monthly Notices of the RAS
\newcommand{\na}{{\it New A}}%
  % New Astronomy
\newcommand{\nar}{{\it New A Rev.}}%
  % New Astronomy Review
%\newcommand{\pra}{{\it Phys.~Rev.~A}}%
          % Physical Review A: General Physics
%\newcommand{\prb}{{\it Phys.~Rev.~B}}%
          % Physical Review B: Solid State
%\newcommand{\prc}{{\it Phys.~Rev.~C}}%
          % Physical Review C
%\newcommand{\prd}{{\it Phys.~Rev.~D}}%
          % Physical Review D
%\newcommand{\pre}{{\it Phys.~Rev.~E}}%
          % Physical Review E
%\newcommand{\prl}{{\it Phys.~Rev.~Lett.}}%
          % Physical Review Letters
\newcommand{\pasa}{{\it PASA}}%
  % Publications of the Astron. Soc. of Australia
%\newcommand{\pasp}{{\it PASP}}%
          % Publications of the ASP
%\newcommand{\pasj}{{\it PASJ}}%
          % Publications of the ASJ
%\newcommand{\qjras}{{\it QJRAS}}%
          % Quarterly Journal of the RAS
\newcommand{\rmxaa}{{\it Rev. Mexicana Astron. Astrofis.}}%
  % Revista Mexicana de Astronomia y Astrofisica
%\newcommand{\skytel}{{\it S\&T}}%
          % Sky and Telescope
%\newcommand{\solphys}{{\it Sol.~Phys.}}%
          % Solar Physics
%\newcommand{\sovast}{{\it Soviet~Ast.}}%
          % Soviet Astronomy
%\newcommand{\ssr}{{\it Space~Sci.~Rev.}}%
          % Space Science Reviews
%\newcommand{\zap}{{\it ZAp}}%
          % Zeitschrift fuer Astrophysik
%\newcommand{\nat}{{\it Nature}}%
          % Nature
%\newcommand{\iaucirc}{{\it IAU~Circ.}}%
          % IAU Cirulars
%\newcommand{\aplett}{{\it Astrophys.~Lett.}}%
          % Astrophysics Letters and Communications
%\newcommand{\apspr}{{\it Astrophys.~Space~Phys.~Res.}}%
          % Astrophysics Space Physics Research
%\newcommand{\bain}{{\it Bull.~Astron.~Inst.~Netherlands}}%
          % Bulletin Astronomical Institute of the Netherlands
%\newcommand{\fcp}{{\it Fund.~Cosmic~Phys.}}%
          % Fundamental Cosmic Physics
%\newcommand{\gca}{{\it Geochim.~Cosmochim.~Acta}}%
          % Geochimica Cosmochimica Acta
%\newcommand{\grl}{{\it Geophys.~Res.~Lett.}}%
          % Geophysics Research Letters
%\newcommand{\jcp}{{\it J.~Chem.~Phys.}}%
          % Journal of Chemical Physics
%\newcommand{\jgr}{{\it J.~Geophys.~Res.}}%
          % Journal of Geophysical Research
%\newcommand{\jqsrt}{{\it J.~Quant.~Spec.~Radiat.~Transf.}}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
%\newcommand{\memsai}{{\it Mem.~Soc.~Astron.~Italiana}}%
          % Mem. Societa Astronomica Italiana
%\newcommand{\nphysa}{{\it Nucl.~Phys.~A}}%
          % Nuclear Physics A
%\newcommand{\physrep}{{\it Phys.~Rep.}}%
          % Physics Reports
%\newcommand{\physscr}{{\it Phys.~Scr}}%
          % Physica Scripta
%\newcommand{\planss}{{\it Planet.~Space~Sci.}}%
          % Planetary Space Science
%\newcommand{\procspie}{{\it Proc.~SPIE}}%
          % Proceedings of the SPIE
